Stochastic Dual Dynamic Programming for Multistage Stochastic Mixed-Integer Nonlinear Optimization

In this paper, we study multistage stochastic mixed-integer nonlinear programs (MS-MINLP). This general class of problems encompasses, as important special cases, multistage stochastic convex optimization with non-Lipschitzian value functions and multistage stochastic mixed-integer linear optimization. We develop stochastic dual dynamic programming (SDDP) type algorithms with nested decomposition, deterministic sampling, and stochastic sampling. The key ingredient is a new type of cuts based on generalized conjugacy. Several interesting classes of MS-MINLP are identified, where the new algorithms are guaranteed to obtain the global optimum without the assumption of complete recourse. This significantly generalizes the classic SDDP algorithms. We also characterize the iteration complexity of the proposed algorithms. In particular, for a $(T+1)$-stage stochastic MINLP with $d$-dimensional state spaces, to obtain an $\epsilon$-optimal root node solution, we prove that the number of iterations of the proposed deterministic sampling algorithm is upper bounded by $\mathcal{O}((\frac{2T}{\epsilon})^d)$, and is lower bounded by $\mathcal{O}((\frac{T}{4\epsilon})^d)$ for the general case or by $\mathcal{O}((\frac{T}{8\epsilon})^{d/2-1})$ for the convex case. This shows that the obtained complexity bounds are rather sharp. It also reveals that the iteration complexity depends polynomially on the number of stages. We further show that the iteration complexity depends linearly on $T$, if all the state spaces are finite sets, or if we seek a $(T\epsilon)$-optimal solution when the state spaces are infinite sets, i.e. allowing the optimality gap to scale with $T$. To the best of our knowledge, this is the first work that reports global optimization algorithms as well as iteration complexity results for solving such a large class of multistage stochastic programs.

==> preamble.tex <==

% control the spacing around section titles
\makeatletter
 \renewcommand\section{\@startsection {section}{1}{\z@}%
     {-4.0mm \@plus -1mm \@minus -.2mm}%
     {1.0mm \@plus.2mm}%
    {\bfseries}}
 \renewcommand\subsection{\@startsection {subsection}{2}{\z@}%
     {-3.0mm \@plus -1mm \@minus -.2mm}%
     {.5mm \@plus.2mm}%
    {}}
 \renewcommand\subsubsection{\@startsection {subsubsection}{3}{\z@}%
     {-2.0mm \@plus -1mm \@minus -.2mm}%
     {.5mm \@plus.2mm}%
    {\itshape}}
% \@startsection {NAME}{LEVEL}{INDENT}{BEFORESKIP}{AFTERSKIP}{STYLE} 
%            optional * [ALTHEADING]{HEADING}
%    Generic command to start a section.  
%    NAME       : e.g., 'subsection'
%    LEVEL      : a number, denoting depth of section -- e.g., chapter=1,
%                 section = 2, etc.  A section number will be printed if
%                 and only if LEVEL gt or eq the value of the secnumdepth
%                 counter.
%    INDENT     : Indentation of heading from left margin
%    BEFORESKIP : Absolute value = skip to leave above the heading.  
%                 If negative, then paragraph indent of text following 
%                 heading is suppressed.
%    AFTERSKIP  : if positive, then skip to leave below heading,
%                       else - skip to leave to right of run-in heading.
%    STYLE      : commands to set style
%  If '*' missing, then increments the counter.  If it is present, then
%  there should be no [ALTHEADING] argument.  A sectioning command
%  is normally defined to \@startsection + its first six arguments.
\makeatother

% \usepackage[compact]{titlesec}

% control the spacing between paragraphs
\setlength{\textfloatsep}{5mm}% Remove \textfloatsep
\setlength{\intextsep}{5mm}% Remove \intextsep
\linespread{0.95}

% for cross reference
% \usepackage{xr}
% \externaldocument{response}

\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{amsmath,amssymb,commath,mathtools,mathrsfs}
\usepackage{dsfont}
\usepackage{wasysym}
\usepackage{bm}
\usepackage{algorithm, algpseudocode, algorithmicx} % 
\algtext*{EndWhile}% Remove "end while" text
\algtext*{EndIf}% Remove "end if" text
\algtext*{EndFor}
\algtext*{EndFunction}
\usepackage{comment}
% \usepackage{subfigure}
% \usepackage{caption}
\usepackage{subcaption}
\captionsetup{compatibility=false}

% create hyperlinks and bookmarks
\usepackage{xr-hyper}
\usepackage[colorlinks=true, 
            linkcolor=blue, 
            urlcolor=black, 
            bookmarksopen=true]{hyperref}
% \usepackage[depth=3]{bookmark}

\usepackage{cases}
\usepackage{empheq}

\setcounter{secnumdepth}{4}

\allowdisplaybreaks

\spnewtheorem{assumption}{Assumption}{\bf}{\it}
\spnewtheorem*{statement}{Statement}{\bf}{\it}

% define math operations and symbols
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\conv}{\mathrm{conv}}
\newcommand{\given}{\,\vert\,}
\renewcommand{\norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\nVert}[1]{\lVert#1\rVert}
\newcommand{\innerprod}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\bangle}[2]{\langle#1,#2\rangle}
\newcommand{\transpose}{\mathsf{T}}
\renewcommand{\square}{\Square}
\newcommand{\cl}{\mathrm{cl}}
\newcommand{\opt}{\mathrm{opt}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\lev}{\mathrm{lev}}
\newcommand{\diam}{\mathrm{diam}\,}
\newcommand{\primal}{\mathrm{prim}}
\newcommand{\reg}{\mathrm{reg}}
\newcommand{\Reg}{\mathrm{R}}
\newcommand{\Fwd}{\mathrm{F}}
\newcommand{\Bwd}{\mathrm{B}}
\newcommand{\Vol}{\mathrm{Vol}}
\newcommand{\Prob}{\mathrm{Prob}}
\renewcommand{\square}{{\scriptsize\Square}}
% define under-bar
\makeatletter
\def\ubar#1{\underline{\sbox\tw@{$#1$}\dp\tw@\z@\box\tw@}}
\makeatother

% define calligraphic and script letters
\makeatletter
% cal capital letters
\def\defcal#1{%
\expandafter\newcommand\csname cal#1\endcsname{\mathcal{#1}}}
\count@=0
\loop
\advance\count@ 1
\edef\y{\@Alph\count@}%
\expandafter\defcal\y
\ifnum\count@<26
\repeat
% scr capital letters
\def\defscr#1{%
\expandafter\newcommand\csname scr#1\endcsname{\mathscr{#1}}}
\count@=0
\loop
\advance\count@ 1
\edef\y{\@Alph\count@}%
\expandafter\defscr\y
\ifnum\count@<26
\repeat
% bb capital letters
\def\defbb#1{%
\expandafter\newcommand\csname bb#1\endcsname{\mathbb{#1}}}
\count@=0
\loop
\advance\count@ 1
\edef\y{\@Alph\count@}%
\expandafter\defbb\y
\ifnum\count@<26
\repeat
\makeatother



% define special math characters
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\renewcommand{\phi}{\varphi}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\tcN}{\tilde{\mathcal{N}}}
\newcommand{\ulQ}{\underline{Q}}
\newcommand{\olQ}{\overline{Q}}
\newcommand{\ulcQ}{\underline{\calQ}}
\newcommand{\olcQ}{\overline{\calQ}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\UB}{\text{\textsc{UpperBound}}}
\newcommand{\LB}{\text{\textsc{LowerBound}}}

\newcommand{\oracle}{\mathrm{oracle}}
\newcommand{\sample}{\mathrm{sample}}

\newcommand{\indfunc}{\mathds{1}}

% define other macros
\def \Re{\mathbb{R}}
\def \Z{\mathbb{Z}}
\def \E{\mathbb{E}}
\def \R{\mathbb{R}}
\def \L{\mathbb{L}}
\def \S{\mathbb{S}}
\def \N{\mathbb{N}}
\def \p{\mathbb{P}}

\def \0{\bm{0}}
\def \a{\bm{a}}
\def \A{\bm{A}}
\def \b{\bm{b}}
\def \B{\bm{B}}
\def \c{\bm{c}}
\def \C{\bm{C}}
\def \d{\bm{d}}
\def \D{\bm{D}}
\def \I{\bm{I}}
\def \M{\bm{M}}
\def \r{\bm{r}}
\def \s{\bm{s}}
\def \u{\bm{u}}
\def \v{\bm{v}}
\def \x{\bm{x}}
\def \y{\bm{y}}
\def \z{\bm{z}}
\def \bxi{\bm{\xi}}

\def \st{\textup{s.t.}}

\def \cF{\mathcal{F}}
\def \cN{\mathcal{N}}
\def \cP{\mathcal{P}}
\def \cQ{\mathcal{Q}}
\def \cT{\mathcal{T}}
\def \cU{\mathcal{U}}
\def \cV{\mathcal{V}}
\def \cX{\mathcal{X}}

\def\lPsi{\underline{\Psi}}
\def\rank{\mathop{\rm rank}}
\def\diag{\mathrm{diag}}
\def\Diag{\mathrm{Diag}}
\def \epi{\mathrm{epi}}


